Mutual Information Based Pilot Design for ISAC

The following paper presents a novel orthogonal pilot design dedicated for \textcolor{black}{integrated sensing and communications (ISAC)} systems performing multi-user communications and target detection. After careful characterization of both sensing and communication metrics based on mutual information (MI), we propose a multi-objective optimization problem (MOOP) tailored for pilot design, dedicated for simultaneously maximizing both sensing and communication MIs. Moreover, the MOOP is further simplified to a single-objective optimization problem, which characterizes trade-offs between sensing and communication performances. Due to the non-convex nature of the optimization problem, we propose to solve it via the projected gradient descent method on the Stiefel manifold. Closed-form gradient expressions are derived, which enable execution of the projected gradient descent algorithm. Furthermore, we prove convergence to a fixed orthogonal pilot matrix. Finally, we demonstrate the capabilities and superiority of the proposed pilot design, and corroborate relevant trade-offs between sensing MI and communication MI. In particular, significant signal-to-noise ratio (SNR) gains for communication are reported, while re-using the same pilots for target detection with significant gains in terms of probability of detection for fixed false-alarm probability. Other interesting findings are reported through simulations, such as an \textit{information overlap} phenomenon, whereby the fruitful ISAC integration can be fully exploited.

==> Actions/R3C7.tex <==
The authors would like to thank the reviewer for the comment.
The convergence analysis proof has been added here for sake of completeness and we do not claim that the main novelty of our work is in the derivations. But, the novelty is the insight we get from it, and not the derivation itself. We have added the following insight in the Introduction instead:
\textcolor{blue}{\input{Actions/insight-convergence}}
We have also removed the following part from the initial version contributions \textit{"..prove that the method can always converge to a stable pilot solution. Convergence properties of the algorithm are derived, as well."}

==> Actions/R3C8.tex <==
We would like to thank the author for the comment.
The results in Fig. \ref{fig:ROC_1} (initially Fig. 6 in the first manuscript) and Fig. \ref{fig:ROC_2} (initially Fig. 7 in the first manuscript) are indeed conducted following Monte Carlo simulations.
In particular, we have generated the \ac{ROC} curves, where each point of probability of detection and probability of false alarm ($P_{\tt{fa}},P_{\tt{d}}$) are obtained via $10^6$ Monte Carlo trials.
In the updated manuscript, we have added the following to emphasize this at the beginning of paragraph \textbf{ROC performance of pilot matrices} in Section \ref{sec:simulations} of the updated manuscript: \textcolor{blue}{\input{Actions/mentioned-ROC-monte-carlo}}

==> sections/algorithm01.tex <==
\begin{algorithm}[H]
\caption{\ac{SCA}-based method to optimize \eqref{eq:problem1}}\label{alg:alg1}
\begin{algorithmic}
\STATE 
\STATE {\textsc{input}: $\pmb{x}_0, \pmb{H}, \pmb{S}$}
\STATE {\textsc{initialize}:} 
\STATE \hspace{0.5cm}  $m=0$,  $\pmb{V}_\ell^{(0)}= \pmb{I}$, $\pmb{W}^{(0)} = \pmb{0}$, $\pmb{p}^{(0)} = \frac{1}{K} \pmb{1}$.
\STATE  {\textsc{while}} $ m < M_{iter}$
\STATE \hspace{0.5cm} Solve $(\mathcal{P}_{1.3}^{(m)})$ in \eqref{eq:problem1_3} to get $\pmb{V}_\ell^{(m+1)},\pmb{W}^{(m+1)}, \pmb{p}^{(m+1)}$.
\STATE \hspace{0.5cm} Update $\pmb{Q}^{(m+1)}$ as $\pmb{Q}^{(m+1)} =\sum\limits_{\ell=1}^L \pmb{V}_\ell^{(m+1)} + \pmb{W}^{(m+1)}$.
\STATE \hspace{0.5cm} Update $\pmb{\Phi}_k^{(m+1)}$ for all $k$ as 
\STATE \hspace{0.5cm} \begin{equation}
	\pmb{\Phi}_k^{(m+1)} = \sum\limits_{\substack{k' = 1 \\ k' \neq k }}^K  p_{k'}^{(m+1)}\pmb{h}_{t,k'}\pmb{h}^H_{t,k'}   +
	 \pmb{C}\pmb{Q}^{(m+1)}\pmb{C}^H + 
	 \pmb{R}_c +
	\sigma_n^2 \pmb{I}
\end{equation}
\STATE \hspace{0.5cm} $m \gets m + 1$
\STATE here..
\STATE \textbf{return}  $\bar{\pmb{x}}^{(M_{{iter}})}$
\end{algorithmic}
\end{algorithm}


==> sections/optimization01-rank1.tex <==
We start by expressing the Lagrangian function of the optimization problem given at iteration $m$ in \eqref{eq:problem1_3}. It can be expressed as
\begin{equation}
	\begin{split}
		&\mathcal{L}(\pmb{V}_1 \ldots \pmb{V}_L ,\pmb{W},\pmb{p} , \pmb{a},\pmb{b}, \pmb{c},\pmb{d},\zeta,\pmb{\Pi}_0 \ldots \pmb{\Pi}_L,\pmb{\pi}) \\ & = -\sum\limits_{\ell = 1}^L\trace(\pmb{\pmb{V}}_\ell) - \trace(\pmb{W}) - \pmb{1}^T \pmb{p} 
		 + 
	\trace(\pmb{\Pi}_0 \pmb{W} )
	+
	\sum\limits_{\ell=1}^L
	\trace(\pmb{\Pi}_\ell \pmb{V}_\ell )
		\\ &
		+ \pmb{\pi}^T \pmb{p}
		+ \sum\limits_{\ell = 1}^L a_\ell\phi_{1,\ell}
		+ \sum\limits_{k = 1}^K b_k\phi_{2,k}
		+ \sum\limits_{p = 1}^P c_p\phi_{3,p}
		\\ &
		+ \sum\limits_{p=1}^P
	      \sum\limits_{k=1}^K d_{p,k}\phi_{4,p,k}
	    + \zeta\phi_{5},
	 \end{split}
\end{equation}
where the  Lagrangian dual variables satisfy $a_\ell \geq 0, b_k \geq 0, c_p \geq 0, d_{p,k} \geq 0 , \zeta \geq 0, \pmb{\Pi}_\ell \succeq \pmb{0}$ for all $\ell,k,p$. The functions $\phi_{1,\ell},\phi_{2,k},\phi_{3,p},\phi_{4,p,k},\phi_5$ are obtained by mapping the constraints in \eqref{eq:problem1_3} under the form $\phi \geq 0$. Due to compact representation, we have omitted the dependence of $\phi$ on the optimization variables and the iteration number $m$. To this extent, we can now define the Lagrange dual function is then defined as follows
\begin{equation}
	\begin{split}
& g(\pmb{a},\pmb{b}, \pmb{c},\pmb{d},\zeta,\pmb{\Pi}_0 \ldots \pmb{\Pi}_L,\pmb{\pi}) 
\\ &= \max\limits_{ \mathcal{S} } \mathcal{L}(\pmb{V}_1 \ldots \pmb{V}_L ,\pmb{W},\pmb{p} , \pmb{a},\pmb{b}, \pmb{c},\pmb{d},\zeta,\pmb{\Pi}_0 \ldots \pmb{\Pi}_L,\pmb{\pi}), 
	\end{split}
\end{equation}
where the set $\mathcal{S}$ is defined as $\mathcal{S} = \lbrace \pmb{V}_\ell \succeq \pmb{0},  \pmb{W} \succeq \pmb{0},  \pmb{p} \geq \pmb{0} \rbrace $.
But since problem $(\mathcal{P}_{1.3}^{(m)})$ is a convex optimization problem with zero duality gap, we can solve the problem via its dual
\begin{equation}
(\mathcal{D}):
	\min\limits_{ \substack{\zeta \geq 0  \\ \lbrace \pmb{a},\pmb{b},\pmb{c},\pmb{d}, \pmb{\pi}  \succeq 0  \rbrace \\ 
							\lbrace \pmb{\Pi}_0 \ldots \pmb{\Pi}_L \succeq 0  \rbrace} } g(\pmb{a},\pmb{b}, \pmb{c},\pmb{d},\zeta,\pmb{\Pi}_0 \ldots \pmb{\Pi}_L,\pmb{\pi}).
\end{equation}
Let the optimal solution of problem $(\mathcal{D})$ as $\pmb{a}^{\opt},\pmb{b}^{\opt}, \pmb{c}^{\opt},\pmb{d}^{\opt},\zeta^{\opt},\pmb{\Pi}_0^{\opt} \ldots \pmb{\Pi}_L^{\opt},\pmb{\pi}^{\opt}$. This means that the optimal $\ell^{th}$ \ac{DL} beamforming matrix, the \ac{AN} covariance matrix, and \ac{UL} power allocation denoted as $\pmb{V}_\ell^{\opt},\pmb{W}^{\opt},\pmb{p}^{\opt}$ also maximizes $\mathcal{L}(\pmb{V}_1 \ldots \pmb{V}_L ,\pmb{W},\pmb{p} ,\pmb{a}^{\opt} \ldots \pmb{\pi}^{\opt}) $, which means that we can find the optimal solution $\pmb{V}_\ell^{\opt}$ by solving the following optimization problem
\begin{equation}
\label{eq:dual-formulation}
\begin{split}
	\max\limits_{  \pmb{V}_\ell \succeq \pmb{0}  }
	\Bigg\lbrace
	&-\trace(\pmb{V}_\ell) 
	+ \frac{a_\ell}{\zeta_{\ell}^{\tt{DL}}}\trace(\pmb{V}_\ell\pmb{H}_{r,\ell})+
	\trace(\pmb{\Pi}_\ell \pmb{V}_\ell)
	\\ &
	- \sum\limits_{p=1}^P 
	 \frac{c_p \vert \alpha_p \vert^2}{\zeta_{p,\tt{DFRC}}^{\tt{Eve}} }
	 \pmb{a}_{N_T}^H(\theta_p)  \pmb{V}_\ell \pmb{a}_{N_T}(\theta_p)
	 \\ &
	+
	 \sum\limits_{p=1}^P
	\sum\limits_{k=1}^K
	d_{p,k}
	\vert \alpha_p \vert^2 \pmb{a}_{N_T}^H(\theta_p)\pmb{V}_\ell\pmb{a}_{N_T}(\theta_p) 
	\\ &
	+
	\zeta\Big( 
	\ISMR_{\tt{max}} \times \trace\Big( \pmb{V}_\ell \pmb{A}_m \Big)
	-
	\trace\Big( \pmb{V}_\ell \pmb{A}_s \Big)
	\Big) 
	  \Bigg\rbrace,
\end{split}
\end{equation}
where terms that are independent of $\pmb{V}_\ell$ are ignored. We can compactly express \eqref{eq:dual-formulation} as follows
\begin{equation}
\label{eq:dual-maximization}
	\max\limits_{  \pmb{V}_\ell \succeq \pmb{0}  }
	\trace(\Phi \pmb{V}_\ell ) 
	-
	\trace \Big\lbrace (\pmb{I} + \pmb{\Gamma} + \zeta^{\opt} \pmb{A}_s) \pmb{V}_\ell  \Big\rbrace,
\end{equation}
where $\Phi = \frac{a_\ell^{\opt}}{\zeta_{\ell}^{\tt{DL}}}\pmb{H}_{r,\ell}
	 + \pmb{\Upsilon} + \zeta^{\opt}\ISMR_{\tt{max}} \pmb{A}_m + \pmb{\Pi}_\ell^{\opt}$, $\pmb{\Upsilon} = \sum\limits_{p=1}^P
	\sum\limits_{k=1}^K
	d_{p,k}^{\opt}
	\vert \alpha_p \vert^2 \pmb{a}_{N_T}(\theta_p)\pmb{a}_{N_T}^H(\theta_p) $ and $\pmb{\Gamma} = \sum\limits_{p=1}^P 
	 \frac{c_p^{\opt} \vert \alpha_p \vert^2}{\zeta_{p,\tt{DFRC}}^{\tt{Eve}} }
	 \pmb{a}_{N_T}(\theta_p)\pmb{a}_{N_T}^H(\theta_p)$. Note that \eqref{eq:dual-maximization} is bounded above due to the semi-positive definiteness of , we prove positive semi definiteness of matrices $\Phi$ and $\pmb{I} + \pmb{\Gamma} + \zeta^{\opt} \pmb{A}_s$. Since $\pmb{I} + \pmb{\Gamma} + \zeta^{\opt} \pmb{A}_s \succeq \pmb{0}$, then there is a unique Hermitian positive definite matrix $\pmb{R}_k^{\frac{1}{2}}$, such that $ \pmb{I} + \pmb{\Gamma} + \zeta^{\opt} \pmb{A}_s = \pmb{R}^{\frac{1}{2}}\pmb{R}^{\frac{1}{2}}$ \cite{horn2012matrix}. Using this square root matrix decomposition, we can express our cost in equation \eqref{eq:dual-maximization} as 
\begin{equation}
	\label{eq:cost-with-sqrt-decom}
	 \max\limits_{  \widetilde{\pmb{V}}_\ell \succeq \pmb{0}  }
	 \trace \Big\lbrace
	  \pmb{R}^{-\frac{1}{2}} \Phi \pmb{R}^{-\frac{1}{2}} \widetilde{\pmb{V}}_\ell 
	  \Big\rbrace
	    -
	 \trace \Big\lbrace \widetilde{\pmb{V}}_\ell \Big\rbrace,
\end{equation} 
where $ \widetilde{\pmb{V}}_\ell = \pmb{R}^{\frac{1}{2}}\pmb{V}_\ell\pmb{R}
^{\frac{1}{2}}$. Now, suppose that the optimal solution, denoted hereby as $\widetilde{\pmb{V}}_\ell^{\opt}$, is not $\rank$-one, i.e. $\rank$ $S > 1$. Then, employing the eigenvalue decomposition, we have that $\widetilde{\pmb{V}}_\ell^{\opt} = \sum\limits_{n=1}^S \beta_n \widetilde{\pmb{v}}_n \widetilde{\pmb{v}}_n^H$ where $\beta_n \geq 0$ and $\Vert \widetilde{\pmb{v}}_n \Vert = 1$, the cost in \eqref{eq:cost-with-sqrt-decom} can be written as
\begin{equation}
\label{eq:cost-with-sqrt-decom-2}
\max\limits_{ \Vert \widetilde{\pmb{v}}_n \Vert = 1  , \beta_n \geq 0 }
	\sum\limits_{n=1}^S
	\beta_n \big( \Vert \Phi^{\frac{1}{2}} \pmb{R}^{-\frac{1}{2}}\widetilde{\pmb{v}}_n \Vert^2 - 1 \big).
\end{equation}
Notice that the cost in \eqref{eq:cost-with-sqrt-decom-2} is upper-bounded as follows
\begin{equation}
\label{eq:cost-with-sqrt-decom-with-eigen}
\begin{split}
&	\sum\limits_{n=1}^S
	\beta_n \big( \Vert \Phi^{\frac{1}{2}} \pmb{R}^{-\frac{1}{2}}\widetilde{\pmb{v}}_n \Vert^2 - 1 \big)
	 \leq  
	\sum\limits_{n=1}^S 
	\beta_n \big( \Vert \Phi^{\frac{1}{2}} \pmb{R}^{-\frac{1}{2}}\widetilde{\pmb{v}}_{\hat{n}} \Vert^2 - 1 \big),
\end{split}
\end{equation} 
where $\Phi^{\frac{1}{2}}$ is the square root decomposition of $\Phi$. Indeed, we have upper bounded all terms of the form $ \Vert \Phi^{\frac{1}{2}} \pmb{R}^{-\frac{1}{2}}\widetilde{\pmb{v}}_n \Vert^2$ by $ \Vert \Phi^{\frac{1}{2}} \pmb{R}^{-\frac{1}{2}}\widetilde{\pmb{v}}_{\hat{n}} \Vert^2$ where $\hat{n} = \argmax\limits_{n = 1 \ldots S} \Vert \Phi^{\frac{1}{2}} \pmb{R}^{-\frac{1}{2}}\widetilde{\pmb{v}}_n \Vert^2 $. But, this bound is achieved by the following $\rank$-one form
\begin{equation}
	\widetilde{\pmb{V}}_\ell^{\rank-1} = \Bigg(\sum\limits_{n=1}^S \beta_n \Bigg) \widetilde{\pmb{v}}_{\hat{n}} \widetilde{\pmb{v}}_{\hat{n}}^H,
\end{equation}
which is a contradiction of the assumption that $S > 1$. Therefore, $\widetilde{\pmb{V}}_\ell^{\opt} $ has to be $\rank$-1 optimal. Now, since we have ${\pmb{V}}_\ell^{\opt} = \pmb{R}^{-\frac{1}{2}}\widetilde{\pmb{V}}_\ell^{\opt}\pmb{R}^{-\frac{1}{2}}$, we must also have that ${\pmb{V}}_\ell^{\opt} $ is $\rank$-one optimal according to $\rank(\pmb{A}\pmb{B}) \leq \min\lbrace \rank(\pmb{A}),\rank(\pmb{B})\rbrace$, which finalizes the proof.
 

%\begin{equation}
%	\begin{split}
%		&\mathcal{L}(\pmb{V}_1 \ldots \pmb{V}_L ,\pmb{W},\pmb{p} , \pmb{a},\pmb{b}, \pmb{c},\pmb{d},\zeta,\pmb{\Pi}_0 \ldots \pmb{\Pi}_L,\pmb{\pi}) \\ & = -\sum\limits_{\ell = 1}^L\trace(\pmb{\pmb{V}}_\ell) - \trace(\pmb{W}) - \pmb{1}^T \pmb{p}
%		\\ &+
%		\sum\limits_{\ell = 1}^L
%		a_\ell
%		\Big(
%		\frac{1}{\zeta_{\ell}^{\tt{DL}}}
%	\trace(\pmb{V}_\ell\pmb{H}_{r,\ell})
%	- \Big(\sum\limits_{\substack{\ell^{'} = 1\\ \ell^{'} \neq \ell}}^L \trace(\pmb{V}_{\ell'}\pmb{H}_{r,\ell}) + 
%	\trace(\pmb{W}\pmb{H}_{r,\ell})  +
%	\sigma_{\ell}^2
%	\Big)
%	\Big)
%	\\ &+ 
%	\sum\limits_{k = 1}^K
%	b_k \Big( 2 p_k \pmb{h}^H_{t,k}
%	[\pmb{\Phi}_k^{(m)}]^{-1}
%	 \pmb{h}_{t,k}
%	 -
%	  \zeta_{k}^{\tt{UL}}
%	  -
%	  p_k^{(m)}
%	  \pmb{h}^H_{t,k}
%	[\pmb{\Phi}_k^{(m)}]^{-1}
%	\pmb{\Phi}_k
%	\pmb{h}^H_{t,k}
%	[\pmb{\Phi}_k^{(m)}]^{-1}
%	\pmb{h}_{t,k}\Big)
%	\\& +
%	\sum\limits_{p=1}^P
%	c_p
%	\Big(
%	\sum\limits_{\substack{k = 1  }}^K p_k \vert g_{k,p} \vert^2 + 
%	\vert \alpha_p \vert^2 \pmb{a}_{N_T}^H(\theta_p)\pmb{W}\pmb{a}_{N_T}(\theta_p)
%	 + \sigma_p^2
%	 -
%	 \frac{1}{\zeta_{p,\tt{DFRC}}^{\tt{Eve}} }
%	\vert \alpha_p \vert^2 \pmb{a}_{N_T}^H(\theta_p)\Big( \sum\limits_{\ell = 1}^L \pmb{V}_\ell \Big)\pmb{a}_{N_T}(\theta_p)
%	\Big)
%	\\& +
%	\sum\limits_{p=1}^P
%	\sum\limits_{k=1}^K
%	d_{p,k}
%	\Big(
%-\frac{1}{\zeta_{p,k}^{\tt{Eve}} }
%	p_k \vert g_{k,p} \vert^2 
%	+
%	\Big(
%	\sum\limits_{\substack{k' = 1 \\ k' \neq k }}^K p_{k'} \vert g_{k',p} \vert^2 + \vert \alpha_p \vert^2 \pmb{a}_{N_T}^H(\theta_p)\pmb{Q}\pmb{a}_{N_T}(\theta_p) + \sigma_p^2
%	\Big)
%	\Big)
%	\\& +
%	\zeta\Big( 
%	\ISMR_{\tt{max}} \times \trace\Big( (\sum\limits_{\ell = 1}^L\pmb{V}_\ell
%	+
%	\pmb{W}) \pmb{A}_m \Big)
%	-
%	\trace\Big( (\sum\limits_{\ell = 1}^L\pmb{V}_\ell
%	+
%	\pmb{W}) \pmb{A}_s \Big)
%	\Big) 
%	\\& + 
%	\trace(\pmb{\Pi}_0 \pmb{W} )
%	+
%	\sum\limits_{\ell=1}^L
%	\trace(\pmb{\Pi}_\ell \pmb{V}_\ell )
%	+
%	\pmb{\pi}^T \pmb{p} ,
%	 \end{split}
%\end{equation}

==> sections/optimization02.tex <==
In the second problem, we deal with
\begin{equation}
 \label{eq:problem2_1}
\begin{aligned}
(\mathcal{P}_2):
\begin{cases}
\max\limits_{\lbrace \substack{ \pmb{U},
									 \pmb{V},  
									 \pmb{W}, 
									  \pmb{p} }  \rbrace}&  \SR_{\tt{
									  DL}} \\
\textrm{s.t.}
 &  \SR_{\tt{UL}} \geq R, \\
 & \trace(\pmb{VV}^H) + \trace(\pmb{W}) + \pmb{1}^T \pmb{p} \leq P_b, \\
& \ISMR \leq \ISMR_{\tt{max}} , \\
& \pmb{W} \succeq \pmb{0},  \ \pmb{p} \succeq \pmb{0}   \\\end{cases}
\end{aligned}
\end{equation}
%%% Replacing the expressions
\begin{equation}
 \label{eq:problem2_2}
\begin{aligned}
(\mathcal{P}_2):
\begin{cases}
\max\limits_{\lbrace \substack{ \pmb{U},
									 \pmb{V},  
									 \pmb{W}, 
									  \pmb{p} }  \rbrace}&  \min_{\ell,p}
	\Big[
	\log_2(1+\SINR_{\ell}^{\tt{DL}})
	-
	\log_2(1+\SINR_{p,\tt{DFRC}}^{\tt{Eve}})
	\Big] \\
\textrm{s.t.}
 &  \min_{k,p}
	\Big[
	\log_2(1+\SINR_{k}^{\tt{UL}})
	-
	\log_2(1+\SINR_{p,k}^{\tt{Eve}})
	\Big] \geq R, \\
 & \trace(\pmb{VV}^H) + \trace(\pmb{W}) + \pmb{1}^T \pmb{p} \leq P_b, \\
& \ISMR \leq \ISMR_{\tt{max}} , \\
& \pmb{W} \succeq \pmb{0},  \ \pmb{p} \succeq \pmb{0}   \\\end{cases}
\end{aligned}
\end{equation}
%% 

\begin{equation}
 \label{eq:problem2_3}
\begin{aligned}
(\mathcal{P}_2):
\begin{cases}
\max\limits_{\Bigg\lbrace \substack{ \pmb{U}\\
									 \pmb{V} \\ 
									 \pmb{W} \\
									  \pmb{p} \\ \theta } \Bigg\rbrace}&  
									  \min_{\ell}
	\Big[
	\log_2(1+\SINR_{\ell}^{\tt{DL}})
	-
	\log_2(1+\theta)
	\Big] \\
\textrm{s.t.}
& \frac
	{\vert \alpha_p \vert^2 \pmb{a}_{N_T}^H(\theta_p)\pmb{VV}^H\pmb{a}_{N_T}(\theta_p)}
	{\sum\limits_{\substack{k = 1  }}^K p_k \vert g_{k,p} \vert^2 + 
	\vert \alpha_p \vert^2 \pmb{a}_{N_T}^H(\theta_p)\pmb{W}\pmb{a}_{N_T}(\theta_p)
	 + \sigma_p^2 } \leq \theta, \ \forall p, \\ 
 &  \min_{k,p}
	\Big[
	\log_2(1+\SINR_{k}^{\tt{UL}})
	-
	\log_2(1+\SINR_{p,k}^{\tt{Eve}})
	\Big] \geq R, \\
 & \trace(\pmb{VV}^H) + \trace(\pmb{W}) + \pmb{1}^T \pmb{p} \leq P_b, \\
& \ISMR \leq \ISMR_{\tt{max}} , \\
& \pmb{W} \succeq \pmb{0},  \ \pmb{p} \succeq \pmb{0}   \\\end{cases}
\end{aligned}
\end{equation}



